A High-Time Resolution Search for Compact Objects using Fast Radio Burst Gravitational Lens Interferometry with CHIME/FRB

The gravitational field of compact objects, such as primordial black holes, can create multiple images of background sources. For transients such as fast radio bursts (FRBs), these multiple images can be resolved in the time domain. Under certain circumstances, these images not only have similar burst morphologies but are also phase-coherent at the electric field level. With a novel dechannelization algorithm and a matched filtering technique, we search for repeated copies of the same electric field waveform in observations of FRBs detected by the FRB backend of the Canadian Hydrogen Mapping Intensity Experiment (CHIME). An interference fringe from a coherent gravitational lensing signal will appear in the time-lag domain as a statistically-significant peak in the time-lag autocorrelation function. We calibrate our statistical significance using telescope data containing no FRB signal. Our dataset consists of $\sim$100-ms long recordings of voltage data from 172 FRB events, dechannelized to 1.25-ns time resolution. This coherent search algorithm allows us to search for gravitational lensing signatures from compact objects in the mass range of $10^{-4}-10^{4} ~\mathrm{M_{\odot}}$. After ruling out an anomalous candidate due to diffractive scintillation, we find no significant detections of gravitational lensing in the 172 FRB events that have been analyzed. In a companion work [Leung, Kader+2022], we interpret the constraints on dark matter from this search.

==> sections/magnification.tex <==
\zarif{This section should only }

%recovery figure

In figure \ref{fig:relmag_v_tau}, we convert the time-lag correlation response into upper limits for the relative magnification ratio as a function of time-lag. For each time-lag bin, we have plotted the largest relative magnification ratio we obtained in that bin. Our bins are logarithimically spaced except for the last bin, which has to extend to the largest time-lag for the dataset, and the lossless region, which has instrumental correlations that affect the correlation statistics (section \ref{sec:compress} for details on the compression algorithm).

\zarif{TODO: Figure \ref{fig:relmag_v_tau} should be public data product figure.}
\begin{figure}[htb!]
    \centering
    \includegraphics[width=0.7\columnwidth]{figures/rel_mag_v_tau.png}
    \caption{The lower limit for relative magnification ratio as a function of time-lag bin for a single FRB event. A lower limit indicates a larger sensitivity to a lensed imaged and is better in this non-detection scenario. The first time-lag bin is dominated by instrumental correlations. Larger time-lag bins include more samples corresponding to an loss in sensitivity for the largest time-lag bin. }
    \label{fig:relmag_v_tau}
\end{figure}

In order to understand the parameter space we probe with our search, observables $\tau$ and $\varepsilon$ need to be converted to the gravitational lensing parameters, the redshift mass, $M_\mathrm{l} (1+ z_\mathrm{l})$, and the normalized impact parameter, $y$. In section \ref{sec:pmobserv}, we detailed how to convert to these parameters. However, we did not characterize limits imposed by observational constraints.

There are four observational constraints that limit the parameter space we probe with our search. First, we cannot identify any lensing time delays below the maximum telescope reflection time, $\sim 300$ ns (section \ref{sec:chimetel}). Building models that capture the effects of telescope reflections is an ongoing goal of CHIME; such models could be used to calibrate future searches. Second, we cannot identify lenses outside the baseband data dump length,  $\sim 1$ ms. Finally, we cannot detect lensing signals below the noise fluctuations. 

Consider that, for a given redshift mass, we explore a range of alignments, quantified by $y$. We want to parameterize, for a given redshift mass, what range of $y$ we probe with a single FRB event. Once these parameters are obtained and combined with other FRB events, it is possible to obtain estimates for the cosmological mass distribution of these compact objects and probability of detection ~\citep{Munoz_paper,frb_lensing_constraint}. This will not be covered in this thesis (This will be covered in a separate analysis (Leung et al., In prep).), however we will describe how we obtain the observational limits, which do not depend on any prior assumptions on these compact objects. 

Let us start with how we obtain $y_\mathrm{max}$ for a given redshift mass. In figure \ref{fig:relmag_v_tau}, we obtain the lower limit on $\varepsilon$ imposed by the null hypothesis, which assumes all observed correlations are not a gravitational lensing signal. We can use the lower limit on $\varepsilon$ and the time range of the time-lag bin to obtain $y_{max}$.
We convert $\varepsilon$ to impact parameter as (Eq.~\ref{eq:impact_conv} in Sec.~\ref{sec:pmobserv})
\begin{equation*}
    y = \sqrt{ |\varepsilon| + |\varepsilon|^{-1} - 2} .
\end{equation*}
We use our lower limit of $\varepsilon$ we obtain $y_{max}$ for every time-lag bin. We now have $y_{max}$, the maximum normalized alignment angle of the lensing system and note that it is independent of mass and the delay. We then use $y_\mathrm{max}$ and the time-lag range and use Eq.~\ref{eq:mass_conv} from section \ref{sec:pmobserv}, 
\begin{equation*}
    M_\mathrm{l} (1+z_\mathrm{l}) = \frac{\tau}{4 G/c^3} \left( \frac{y}{2} \sqrt{ y^2 +4}  - \ln \left( \frac{ y + \sqrt{ y^2 +4}} {y - \sqrt{ y^2 +4}} \right)  \right)^{-1} ,
\end{equation*}
where $\tau$ is either the start or end of the time-lag bin, to obtain the upper observable limit of $y$ as a function of redshift mass. This can be seen as the top most edge in figure \ref{fig:y_vs_mass}.

In order to obtain the lower observable limit, first consider our minimum time observable time delay, 300 ns. We want to find the minimum observable alignment angle, which implies we are in the limit where $y<<1$. We can approximate $\tau$,
\begin{equation*}
    \tau = \frac{4 G M_\mathrm{l}(1+ z_\mathrm{l})}{ c^3} \bigg( \frac{1}{2} y\sqrt{ y^2 +4}  + \ln \bigg( \frac{ \sqrt{ y^2 +4}+y} {\sqrt{ y^2 +4}-y} \bigg) \bigg) ,
\end{equation*}
in this limit to obtain
\begin{equation*}
    \tau = \frac{4 G M_\mathrm{l}(1+ z_\mathrm{l})}{ c^3}  y~.
\end{equation*}
Then, for a given redshift mass and the minimum $\tau_\mathrm{min} = 300 ~ns$, we have
\begin{equation*}
     y_{min}  = \frac{4 G M_\mathrm{l}(1+ z_\mathrm{l})}{ \tau_\mathrm{min} c^3} .
\end{equation*}
This is represented as the bottom edge of the shaded region in figure \ref{fig:y_vs_mass}.

Figure \ref{fig:y_vs_mass} highlights an example of the parameter space we can probe with one FRB event, as the shaded region, and where it is possible to assert a null detection. The collection of these parameters for all our events then implies limits on the existence of gravitational lensing objects within the line of sight of the FRBs that have been detected. We further note that masses larger than this range become degenerate in detection. In order to produce time delays on the order of our search range, higher mass objects would need $y<<1$ which would produce images that have $\varepsilon \sim 1$. Nonetheless, it is possible to detect images from larger mass compact objects, while not being able to recover the mass of the lens in this scenario. 

In this section, we have provided the parameter space across which we can assert a non-detection. However, note we have not characterized any decoherence effects. In figure \ref{fig:y_vs_mass}, we show the parameter space that can be explored with an FRB event. The absence of a time-lag image detection would allow us to assert that there is not a gravitational lens along this line of sight.

\zarif{TODO: Figure \ref{fig:y_vs_mass} should be made from public data product.}

\begin{figure}[htb!]
    \centering
    \includegraphics[width=0.7\columnwidth]{figures/impact_v_mass.png}
    \caption{The parameter space of impact parameter and lensing mass we have searched using a single FRB. The shaded region indicates the parameter space where it is possible to assert a null detection.} 
    \label{fig:y_vs_mass}
\end{figure}

==> sections/rf.tex <==
We autocorrelate $\approx 200$ FRBs detected by CHIME FRB with different dispersion measures and brightnesses, measuring $R_f(\tau)$ for each independent sightline. Our correlation algorithm~\cite{CHIME2021Lensing} measures the delay spectrum of the noise-whitened electric field signal $E(t)$ : 

$$G(\tau) = \sum_t E(t) E(t + \tau) W(t)$$

where $W(t)$ is a positive-valued SNR matched filter approximately tuned to duration of the burst.
It can be shown that after subtracting the system temperature correlating with itself at $\tau = 0$, the minimum detectable flux ratio is 
\begin{equation}
    R_f(\tau) = |G(\tau) / G(0)|^2 + \mathcal{O}(|G(\tau) /  G(0)|^4) < 1
\end{equation}
under the assumption that there is only one lensed image, and that most of the fluctuations in $G(\tau)$ are due to noise variance.\footnote{In contrast to Refs.~\citep{munoz2016lensing,sammons2020first}, we adopt the sign convention that brighter image is in the denonimator, i.e., that $R_f \leq 1$.}
%The whitened, band-integrated ``flux'' as a function of time can be written $E^2(t)$, and the fluence can be measured by summing over time samples. -pipeline
%To improve the sensitivity of the correlation, we also use a window function to exploit the temporal structure of the FRB. After coherent de-dispersion and RFI removal in baseband space, we construct the window function by summing over channels and smoothing the resulting light curve with a Gaussian whose width $\sigma$ is set by the variability timescale of the FRB. Finally, the autocorrelation code
%computes

$$G(\tau) = \sum_t E(t) E(t + \tau) W(t)$$

as a function of trial delay $\tau$. From the correlator output we can extract the magnification ratio as a function of lag. This conversion is done as follows. We first define the quantity
%
$$S_W(\tau) = \sum_t E^2(t) W(t + \tau).$$
%
and choose the normalization of $W$ such that $S_W(0)$ is the fluence of the burst. We call this quantity the lag-fluence. It is equivalent to the fluence at zero lag, where it is at its maximum, but as $\tau$ increases the window gets misaligned with the light curve $S_W(\tau)$ decreases. Eventually the window moves to delays longer than the pulse duration, and $S_W(\tau) \to 0$.
Our correlator computes 
%
$$G(\tau) = \sum_t E(t) E(t + \tau) W(t).$$
%
Suppose that the timestream $E(t)$ contains a second image corresponding to a putative lens signal, with a flux magnification ratio of $\epsilon^2 < 1$. In the regime of coherent lensing (see Section~\ref{sec:decoherence}), semiclassical (or eikonal~\cite{jow2020wave}) optics allows us to model the electric field from the second image as $E'(t) = \epsilon E(t - \tau_{lens})$. In this limit, $E'$ and $E$ correlate with each other when they are temporally aligned $(\tau = \tau_{lens})$, yielding a peak in the autocorrelation function of magnitude
%
$$G(\tau_{lens}) = \epsilon S_W(0)$$
%
The autocorrelation peak at zero lag is boosted as well. After subtracting the background from the system temperature, the zero lag peak height is
$$G(0) = S_W(0) + \epsilon^2 S_W(\tau_{lens})$$
We calculate
$$\mathcal{R}(\tau) = G(\tau) / G(0) = \dfrac{\epsilon}{1 + \epsilon^2 S_W(\tau_{lens})/S_W(0)}.$$
%
Solving for $\epsilon$ gives us 
$$
\epsilon(\tau) = 
\begin{cases}
    \dfrac{S_W(0)}{S_W(\tau_{lens})\mathcal{R}(\tau)} - \mathcal{R}(\tau) - 2\mathcal{R}(\tau)^3\dfrac{S_W(\tau_{lens})}{S_W(0)} \\ \mathcal{R}(\tau) + 2 \dfrac{S_W(\tau_{lens})}{S_W(0)} \mathcal{R}(\tau)^3 
\end{cases}
$$

The former solution is unphysical and diverges as $S_W(\tau_{lens}),\mathcal{R}(\tau) \to 0$. Furthermore, for lags larger than a few nanoseconds, $|\mathcal{R}(\tau)| < 0.05$, making the $\mathcal{R}^3$ term negligible. Thus the lens magnification ratio is to leading order
%
$$\epsilon^2 = |G(\tau) / G(0)|^2 + \mathcal{O}(|G(\tau) / G(0)|^4).$$
%
